Object-level Scene Deocclusion

Deoccluding the hidden portions of objects in a scene is a formidable task, particularly when addressing real-world scenes. In this paper, we present a new self-supervised PArallel visible-to-COmplete diffusion framework, named PACO, a foundation model for object-level scene deocclusion. Leveraging the rich prior of pre-trained models, we first design the parallel variational autoencoder, which produces a full-view feature map that simultaneously encodes multiple complete objects, and the visible-to-complete latent generator, which learns to implicitly predict the full-view feature map from partial-view feature map and text prompts extracted from the incomplete objects in the input image. To train PACO, we create a large-scale dataset with 500k samples to enable self-supervised learning, avoiding tedious annotations of the amodal masks and occluded regions. At inference, we devise a layer-wise deocclusion strategy to improve efficiency while maintaining the deocclusion quality. Extensive experiments on COCOA and various real-world scenes demonstrate the superior capability of PACO for scene deocclusion, surpassing the state of the arts by a large margin. Our method can also be extended to cross-domain scenes and novel categories that are not covered by the training set. Further, we demonstrate the deocclusion applicability of PACO in single-view 3D scene reconstruction and object recomposition.

==> limitation.tex <==
\section{Limitations}


Despite the superior performance of our approach, there are still some limitations in this work. 

First, our approach is struggling to handle shadows on the objects. For instance, in the bottom right image of Figure 6 in this supplementary file, the completed skiboard has some black artifacts due to the shadow of the skier projected on it. In addition, the shadow on the background image may limit our image recomposition application, since the recomposed scene may have inconsistencies of shadows with the given image. How to deal with shadows in the deocclusion task remains an open problem for future research. 


Second, our approach requires a high-quality segment map and text annotation of each object as pre-processing. Although they can be acquired with foundation models like SAM~\cite{kirillov2023segment} and GPT-4V~\cite{openai2023gpt4v}, respectively, such requirements still hinder the automation of our pipeline on images without such annotation. In addition, our performance is limited by the quality of the segmentation map. 

Third, our pipeline is not ready to handle the object partially exceeding the image boundary. For instance, in the top right image of Figure 4 in this supplementary file, our approach does not deocclude the left side of this teddy bear since it exceeds the left boundary of the image. One solution to complete this teddy bear is to pad a border with the proper size on the top left boundary of the image; yet, it requires additional pre-processing by the user.  


In addition, our approach focuses on the object-level deocclusion and leaves the background region deocclusion for existing inpainting models, e.g., LAMA~\cite{suvorov2022resolution}. Thus, the background quality in our image recomposition application is limited by such models. 



Also, the lack of 3D awareness can lead to unreasonable deocclusion results. For example, in the bottom right image of Figure 8, the banana and the two sandwiches occupy a shared 3D space, which is unreasonable in practice. The 3D-aware object-level scene deocclusion can be a potential research direction in the future.  

